When Do We Need Graph Neural Networks for Node Classification?

Graph Neural Networks (GNNs) extend basic Neural Networks (NNs) by additionally making use of graph structure based on the relational inductive bias (edge bias), rather than treating the nodes as collections of independent and identically distributed (i.i.d.) samples. Though GNNs are believed to outperform basic NNs in real-world tasks, it is found that in some cases, GNNs have little performance gain or even underperform graph-agnostic NNs. To identify these cases, based on graph signal processing and statistical hypothesis testing, we propose two measures which analyze the cases in which the edge bias in features and labels does not provide advantages. Based on the measures, a threshold value can be given to predict the potential performance advantages of graph-aware models over graph-agnostic models.

==> env.tex <==
% \documentclass{article}
% \usepackage{geometry}
% \geometry{left=3cm,right=3cm,top=2cm,bottom=2cm}

%File: formatting-instruction.tex
\usepackage{amssymb,bm,amsthm}
\usepackage{enumerate}
\usepackage{color, colortbl}
\usepackage{booktabs, multirow}
\definecolor{darkgreen}{rgb}{0, 0.5, 0}
\definecolor{red}{rgb}{1, 0, 0}
\definecolor{purple}{rgb}{0.5, 0, 0.5}
\usepackage{chngpage}
% \usepackage{subfigure}
\usepackage{comment}
\usepackage{mfirstuc}
\usepackage{mathtools}
\usepackage{lettrine}
\usepackage{pxfonts}
\def\UrlBreaks{\do\/\do-}


\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}

\newcommand\etal{\textit{et al.}}
\newcommand\ie{\textit{i.e.}}
\newcommand\eg{\textit{e.g.,}}
\newcommand\st{\textit{s.t.}}
\newcommand\wrt{\textit{w.r.t.}}
\newcommand\etc{\textit{etc.}}
\newcommand\iid{\textit{i.i.d.}}
\newcommand\doubleE{\mathbb{E}}
\newcommand\doubleP{\mathbb{P}}
\newcommand\doubleR{\mathbb{R}}
\newcommand\scriptS{\mathcal{S}}
\newcommand\scriptE{\mathcal{E}}
\newcommand\scriptO{\mathcal{O}}
\newcommand\scriptA{\mathcal{A}}
\newcommand\scriptX{\mathcal{X}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\red}{\textcolor{red}}


% Equations:
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqnn}{\begin{equation*}}
\newcommand{\eeqnn}{\end{equation*}}
\newcommand{\beqy}{\begin{eqnarray}}
\newcommand{\eeqy}{\end{eqnarray}}
\newcommand{\beqynn}{\begin{eqnarray*}}
\newcommand{\eeqynn}{\end{eqnarray*}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bex}{\begin{example}}
\newcommand{\eex}{\end{example}}
\newcommand{\trace}{\mathrm{trace}}
% Algorithm

\newcommand{\balg}[1]{\begin{algorithm} \caption{#1}}
\newcommand{\ealg}{\end{algorithm}}

\newcommand{\balgc}{\begin{algorithmic}[1]}
\newcommand{\ealgc}{\end{algorithmic}}

% Arrays, Matrices and Tables:
\newcommand{\bary}{\begin{array}}
\newcommand{\eary}{\end{array}}
\newcommand{\bmx}{\begin{bmatrix}}
\newcommand{\emx}{\end{bmatrix}}
\newcommand{\bsmx}{\left[\begin{smallmatrix}}
\newcommand{\esmx}{\end{smallmatrix}\right]}
\newcommand{\bmxc}[1]{\left[\begin{array}{@{}#1@{}}}
\newcommand{\emxc}{\end{array}\right]}
%position
\newcommand{\bcn}{\begin{center}}
\newcommand{\ecn}{\end{center}}

% To give an extra space above say \bar{b} under an hline:
\newcommand{\clear}[1]{\mathrel{\raisebox{-.50ex}{$#1$}}}
% use (on the matrix row following the \hline):  \clear{\bar{b}}
% or just use: \mathrel{\raisebox{-.75ex}{$\bar{b}$}}

% Operations:
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\ReLU}{\mathrm{ReLU}}
\newcommand{\bTReLU}{\mathrm{bTReLU}}
\newcommand{\sgn}{\mathrm{sgn}}
\renewcommand{\vec}{\mathrm{vec}}
 


%Dimension of matrices:
 
\newcommand{\cve}[1]{{#1 \times 1}}
 
\newcommand{\Rbb}{{\mathbb{R}}}
\newcommand{\Zbb}{{\mathbb{Z}}}
\newcommand{\Cbb}{{\mathbb{C}}}

%\newcommand{\kbk}{{k \times k}}
\newcommand{\nbk}{{n \times k}}
\newcommand{\nbn}{{n \times n}}
\newcommand{\nbm}{{n \times m}}
\newcommand{\nbp}{{n \times p}}
\newcommand{\mbm}{{m \times m}}
\newcommand{\mbn}{{m \times n}}
\newcommand{\mbp}{{m \times p}}
\newcommand{\pbn}{{p \times n}}
\newcommand{\pbp}{{p \times p}}
\newcommand{\mbmmn}{{m \times (m-n)}}
\newcommand{\bigO}{{\mathcal{O}}}

\newcommand{\Rk}{\Rbb^{k}}
\newcommand{\Rm}{\Rbb^{m}}
\newcommand{\Rn}{\Rbb^{n}}
\newcommand{\Rp}{\Rbb^{p}}
\newcommand{\Rkbk}{\Rbb^{k \times k}}
\newcommand{\Rnbk}{\Rbb^{n \times k}}
\newcommand{\Rnbn}{\Rbb^{n \times n}}
\newcommand{\Rnbm}{\Rbb^{n \times m}}
\newcommand{\Rnbp}{\Rbb^{n \times p}}
\newcommand{\Rmbm}{\Rbb^{m \times m}}
\newcommand{\Rmbn}{\Rbb^{m \times n}}
\newcommand{\Rmbp}{\Rbb^{m \times p}}
\newcommand{\Rpbn}{\Rbb^{p \times n}}
\newcommand{\Rpbm}{\Rbb^{p \times m}}
\newcommand{\Rpbp}{\Rbb^{p \times p}}
\newcommand{\Rmbmmn}{\Rbb^{m \times (m-n)}}
\newcommand{\Cn}{\Cbb^{n}}
\newcommand{\Cmbn}{\Cbb^{m\times n}}
\newcommand{\Zm}{\Zbb^{m}}
\newcommand{\Zn}{\Zbb^{n}}
\newcommand{\Zmbn}{\Zbb^{m \times n}}
\newcommand{\Znbn}{\Zbb^{n \times n}}


% Statistical Material:
\newcommand{\pro}[1]{\mathcal{P}\{ #1 \} }
\newcommand{\Exp}[1]{\mathcal{E}\{ #1 \} }
\newcommand{\cov}[1]{\mathrm{cov}\{#1\}}
\newcommand{\cnd}{\kappa}

% Special symbols:

\newcommand{\sE}{{\scriptscriptstyle E}}
\newcommand{\sss}{\scriptscriptstyle }
\newcommand{\sLS}{{\scriptscriptstyle \text{LS}}}
\newcommand{\sILS}{{\scriptscriptstyle \text{ILS}}}
\newcommand{\sRLS}{{\scriptscriptstyle \text{RLS}}}
\newcommand{\sOL}{{\scriptscriptstyle \text{OL}}}
\newcommand{\sOB}{{\scriptscriptstyle \text{OB}}}
\newcommand{\sOR}{{\scriptscriptstyle \text{OR}}}
\newcommand{\sBB}{{\scriptscriptstyle \text{BB}}}
\newcommand{\sBR}{{\scriptscriptstyle \text{BR}}}
\newcommand{\sBL}{{\scriptscriptstyle \text{BL}}}
\newcommand{\sBBL}{{\scriptscriptstyle \text{BBL}}}
\newcommand{\sBBS}{{\scriptscriptstyle \text{BBS}}}
\newcommand{\sBBV}{{\scriptscriptstyle \text{BBV}}}
\newcommand{\sBBBD}{{\scriptscriptstyle \text{BBBD}}}
\newcommand{\sOBL}{{\scriptscriptstyle \text{OBL}}}
\newcommand{\sOBS}{{\scriptscriptstyle \text{OBS}}}
\newcommand{\sOBV}{{\scriptscriptstyle \text{OBV}}}
\newcommand{\sOBBD}{{\scriptscriptstyle \text{OBBD}}}


\newcommand{\mbbR}{{\mathbb{R}}}
\newcommand{\mbbZ}{{\mathbb{Z}}}

%Bold
\newcommand{\A}{\boldsymbol{A}}
\newcommand{\B}{\boldsymbol{B}}
\newcommand{\C}{\boldsymbol{C}}
\newcommand{\D}{\boldsymbol{D}}
\newcommand{\F}{\boldsymbol{F}}
\newcommand{\G}{\boldsymbol{G}}
\renewcommand{\H}{\boldsymbol{H}}
\newcommand{\I}{\boldsymbol{I}}
\newcommand{\J}{\boldsymbol{J}}
\newcommand{\K}{\boldsymbol{K}}
\renewcommand{\L}{\boldsymbol{L}}
\newcommand{\M}{\boldsymbol{M}}
\newcommand{\N}{\boldsymbol{N}}
\renewcommand{\P}{\boldsymbol{P}}
\newcommand{\Q}{\boldsymbol{Q}}
\renewcommand{\S}{\boldsymbol{S}}
\newcommand{\T}{\boldsymbol{T}}
\newcommand{\U}{\boldsymbol{U}}
\newcommand{\V}{\boldsymbol{V}}
\newcommand{\W}{\boldsymbol{W}}
\newcommand{\X}{{\boldsymbol{X}}}
\newcommand{\Y}{{\boldsymbol{Y}}}
\newcommand{\Z}{\boldsymbol{Z}}
\renewcommand{\a}{\boldsymbol{a}}
\renewcommand{\b}{\boldsymbol{b}}
\renewcommand{\c}{\boldsymbol{c}}
\renewcommand{\d}{\boldsymbol{d}}
\newcommand{\e}{\boldsymbol{e}}
\newcommand{\f}{\boldsymbol{f}}
\newcommand{\g}{\boldsymbol{g}}
\newcommand{\h}{\boldsymbol{h}}
\renewcommand{\l}{\boldsymbol{l}}
\newcommand{\n}{\boldsymbol{n}}
\newcommand{\p}{\boldsymbol{p}}
\newcommand{\q}{\boldsymbol{q}}
% We have to define bold r in the following way, otherwise there would be a problem
\newcommand{\s}{\boldsymbol{s}}
\renewcommand{\u}{\boldsymbol{u}}
\renewcommand{\v}{\boldsymbol{v}}
\newcommand{\w}{\boldsymbol{w}}
\newcommand{\x}{{\boldsymbol{x}}}
\newcommand{\y}{{\boldsymbol{y}}}
\newcommand{\z}{\boldsymbol{z}}
\newcommand{\0}{{\boldsymbol{0}}}

%bar
\newcommand{\bd}{{\bar{d}}}
\newcommand{\bl}{{\bar{l}}}
\newcommand{\bx}{{\bar{x}}}
\newcommand{\by}{{\bar{y}}}
\newcommand{\bz}{{\bar{z}}}
\newcommand{\bc}{{\bar{c}}}
\newcommand{\br}{{\bar{r}}}
%barbold

\newcommand{\bbz}{{\bar{\z}}}
\newcommand{\bby}{{\bar{\y}}}
\newcommand{\bbx}{{\bar{\x}}}
\newcommand{\bbL}{{\bar{\L}}}
\newcommand{\bbD}{{\bar{\D}}}
\newcommand{\bbQ}{{\bar{\Q}}}
\newcommand{\bbR}{{\bar{\R}}}
\newcommand{\bbu}{{\bar{\u}}}
\newcommand{\bbl}{{\bar{\l}}}

%tilde
\newcommand{\td}{{\tilde{d}}}
\newcommand{\tr}{{\tilde{r}}}
\newcommand{\tv}{{\tilde{v}}}
\newcommand{\ty}{{\tilde{y}}}

%tildebold
\newcommand{\tbD}{{\tilde{\D}}}
\newcommand{\tbL}{{\tilde{\L}}}
\newcommand{\tbP}{{\tilde{\P}}}
\newcommand{\tbQ}{{\tilde{\Q}}}
\newcommand{\tbl}{{\tilde{\l}}}
\newcommand{\tbR}{{\tilde{\R}}}
\newcommand{\tby}{{\tilde{\y}}}

%check
\newcommand{\cba}{{\check{\a}}}
\newcommand{\cbx}{{\check{\x}}}
\newcommand{\cbz}{{\check{\z}}}

%hat
\newcommand{\ha}{{\hat{a}}}
\newcommand{\hr}{{\hat{r}}}
\newcommand{\hx}{{\hat{x}}}
\newcommand{\hz}{{\hat{z}}}
%hatbold
\newcommand{\hbG}{{\hat{\G}}}
\newcommand{\hbR}{{\hat{\R}}}
\newcommand{\hba}{{\hat{\a}}}
\newcommand{\hbc}{{\hat{\c}}}
\newcommand{\hbd}{{\hat{\d}}}
\newcommand{\hbr}{{\hat{\r}}}
\newcommand{\hbw}{{\hat{\w}}}
\newcommand{\hbx}{{\hat{\x}}}
\newcommand{\hby}{{\hat{\y}}}
\newcommand{\hbz}{{\hat{\z}}}


% Special format:
\newcommand{\bSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\fnl}{{\mathcal{F}}}
\newcommand{\huber}{{\mathcal{H}}}
\newcommand{\6}{{\partial}}
\newcommand{\8}{{\infty}}
\newcommand{\4}{{\nabla}}

%functions
\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\round}[1]{\lfloor#1\rceil}
\providecommand{\rnd}[1]{\lfloor #1 \rceil}
\providecommand{\abs}[1]{\left| #1 \right|}

\newcommand{\colvec}[2][1]{%
\scalebox{#1}{%
\renewcommand{\arraystretch}{1.45}%
$\begin{bmatrix}#2\end{bmatrix}$%
}}

